Simultaneous Near-Field THz Communications and Sensing with Full Duplex Metasurface Transceivers

In this paper, a Full Duplex (FD) eXtremely Large (XL) Multiple-Input Multiple-Output (MIMO) node equipped with reconfigurable metasurface antennas at its transmission and reception sides is considered, which is optimized for simultaneous multi-user communications and sensing in the near-field regime at THz frequencies. We first present a novel Position Error Bound (PEB) analysis for the spatial parameters of multiple targets in the vicinity of the FD node, via the received backscattered data signals, and devise an optimization framework for its metasurface-based precoder and combiner. Then, we formulate and solve an optimization problem aiming at the downlink sum-rate maximization, while simultaneously ensuring a minimum PEB requirement for targets' localization. Our simulation results for a sub-THz system setup validate the joint near-field communications and sensing capability of the proposed FD XL MIMO scheme with metasurfaces antennas, showcasing the interplay of its various design parameters.

==> Poster_SPAWC_Source_Files/format.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% some definitions from R. Fischer's template
\def\bbbr{{\sf I\!R}} %reelle Zahlen
\def\bbbn{{\sf I\!N}} %natuerliche Zahlen
\def\bbbf{{\sf I\!F}} %finiter K"orper

\def\R{\bbbr}
\def\Z{\bbbz}
\def\N{\bbbn}
\def\C{\bbbc}
\def\Q{\bbbq}
\def\F{\bbbf}

\def\ve#1{{\mathchoice{\mbox{\boldmath$\displaystyle #1$}}%
              {\mbox{\boldmath$\textstyle #1$}}%
              {\mbox{\boldmath$\scriptstyle #1$}}%
              {\mbox{\boldmath$\scriptscriptstyle #1$}}}}

%%%% Laengen %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unitlength1cm
\setcounter{secnumdepth}{5}
\setcounter{tocdepth}{5}
\textwidth=17cm
\textheight=23.5cm
\hoffset=-20mm
%\voffset=-10mm
\parindent0cm
\parskip.5em plus.1em minus .2em
\headheight6mm
\headsep8mm
\footskip22mm
\oddsidemargin16.0mm
\evensidemargin11.5mm
\renewcommand{\baselinestretch}{1.1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% commands
\renewcommand{\R}{\mathbb{R}}
\renewcommand{\Z}{\mathbb{Z}}
\renewcommand{\N}{\mathbb{N}}
\renewcommand{\C}{\mathbb{C}}
\renewcommand{\Q}{\mathbb{Q}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Poster_SPAWC_Source_Files/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                      Makros & Definitionen                           %
%                    Globale Datei 'macros.tex'                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%========= Schriftgr\"{o}{\ss}en im mathematischen Modus
\newcommand{\dis}{\displaystyle}
\newcommand{\scs}{\scriptstyle}
\newcommand{\scscs}{\scriptscriptstyle}
\newcommand{\txs}{\textstyle}
%========= Symbolgr\"{o}{\ss}en im mathematischen Modus
%\big \Big \bigg \Bigg
%========= Schriftgr\"{o}{\ss}en im Textmodus
%\tiny
%\scriptsize
%\footnotesize
%\small
%\normalsize
%\large
%\Large
%\LARGE
%\huge
%\Huge

\newcommand{\psfragfs}{0.6}

%========= Umgebungen
\newcommand{\er}{\mathrm{e}} % Euler'sche Zahl in roman
\newcommand{\wtvarphi}{\widetilde{\varphi}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\ovl}[1]{\overline{#1}}
\newcommand{\ovlsup}[2]{\overline{#1 ^{ #2 }}}
\newcommand{\cm}{\check{m}}
\newcommand{\brarray}[2]{\left[\!\! \begin{array}{#1} #2 \end{array} \!\! \right]} % eckige Klammern um array
\newcommand{\barray}[2]{\begin{array}{#1} #2 \end{array} } % keine Klammern um array
\newcommand{\mpage}[3]{\begin{minipage}[#1]{#2} #3 \end{minipage}} % minipage-Umgebung: #1: position, #2: width, #3: text
\newcommand{\centr}[1]{\begin{center} #1 \end{center}} % center-Umgebung: #1: text
\newcommand{\accolade}[1]{\left\{#1\right\}} % Alt!!!
\newcommand{\abrackets}[1]{\left\{#1\right\}}
\newcommand{\leftbracket}[2]{\left\{\begin{array}{#1} #2 \end{array} \right.}
\newcommand{\Ztr}[1]{\mathcal{Z} \left\{#1\right\}}
\newcommand{\IZtr}[1]{\mathcal{Z}^{-1} \!\! \left\{#1\right\}}
\newcommand{\trsp}{T}                  % transponiert
%\newcommand{\hermitsch}{{\mathrm{\scriptsize H}}}             % hermitsch
\newcommand{\hermitsch}{H}             % hermitsch
\newcommand{\frob}{{{\scriptsize F}}}             % Frobenius-F
\newcommand{\trace}[1]{\mathrm{tr}\{#1\}}
\newcommand{\Q}[1]{\mathrm{Q}\left( #1 \right)}  % Q-function
\newcommand{\expect}[1]{{E}\!\left\{ #1 \right\}}                   % Erwartungwert
\newcommand{\Expect}{{E}}         % Erwartungwert
\newcommand{\expectind}[2]{{E}_{#1}\!\left\{ #2 \right\}}     % Erwartungwert + Index
\newcommand{\real}[1]{\Re \left\{ #1 \right\}}              % Realteil
\newcommand{\imag}[1]{\Im \left\{#1 \right\}}               % Imagin\"{a}rteil
%\newcommand{\degrees}[1]{\ensuremath{#1^\circ}}             % Grad
\newcommand{\vecOp}[1]{\mathrm{{vec}} \! \left( #1 \right)}      % vec-Operator
\newcommand{\sqrtm}[1]{{#1^{1/2}}}      % Wurzel einer Matrix
\newcommand{\sqrtmt}[1]{{(#1^{1/2})^{\trsp}}}      % Wurzel einer Matrix transponiert
\newcommand{\sqrtmh}[1]{{(#1^{1/2})^{\hermitsch}}} % Wurzel einer Matrix hermitsch
\newcommand{\round}[1]{\lceil #1 \rfloor}      % Rundungsoperator
\newcommand{\roundU}[1]{\lceil #1 \rceil}      % Aufrundungsoperator
\newcommand{\roundD}[1]{\lfloor #1 \rfloor}    % Abrundungsoperator
\newcommand{\conv}{\ast}    % Faltungsoperator

\newcommand{\equbr}[1]{(\ref{#1})}

%========= Operatoren
\renewcommand{\Re}{\ensuremath{\operatorname{Re}}}
\renewcommand{\Im}{\ensuremath{\operatorname{Im}}}


%========= Definitionen
\newcommand{\sigko}{{\cal A}}               % Signalkonstellation
\newcommand{\sigkoCCK}{{\cal C}}            % CCK Signalkonstellation
\newcommand{\Nnull}{{\cal N}_0}             % Rauschleistungsdichte N_0
\newcommand{\qh}{q_{h}}                     % Kanalged\"{a}chtnis scalares-FIR Filter
\newcommand{\qbt}{\widetilde{q}_{b}}        % Kanalged\"{a}chtnis scalares-FIR Filter
%\newcommand{\qht}{\widetilde{q}_h}          % Kanalged\"{a}chtnis matrix-FIR Filter
\newcommand{\qht}{Q_h}          % Kanalged\"{a}chtnis matrix-FIR Filter
\newcommand{\qtrt}{\widetilde{q}_{tr}}      % Kanalged\"{a}chtnis truncated
\newcommand{\dmin}{d_{\mathrm{\footnotesize min}}}% minimale euklidische Distanz
\newcommand{\var}{\sigma^2}                 % Varianz
\newcommand{\hypo}[1]{\check{#1}}           % Hypothese
\newcommand{\dec}[1]{\hat{#1}}              % Entscheidung
\newcommand{\ntx}{N_T}                      % Anzahl Sendeantennen
\newcommand{\itr}{n_t}                      % Index Sendeantennen
\newcommand{\nrx}{N_R}                      % Anzahl Empangsantennen
\newcommand{\ire}{n_r}                      % Index Empfangsantennen
\newcommand{\nST}{N_\mathrm{ST}}            % Anzahl Ausgaenge eines ST CODES
\newcommand{\iST}{n_\mathrm{ST}}            % Index Ausgaenge eines ST CODES
\newcommand{\nG}{N_\mathrm{G}}              % Anzahl Filtervektoren
\newcommand{\iG}{n_\mathrm{g}}              % Index Filtervektoren


\newcommand{\ig}{n_g}

\newcommand{\diag}[1]{{{\rm diag} \left( #1 \right) }}        % CIR

\newcommand{\Quant}[1]{\mathcal{Q}\{ #1 \}} % Quantizer operation

\newcommand{\dB}{\mathrm{dB}}                  % dB
\newcommand{\Hz}{\mathrm{Hz}}
\newcommand{\kHz}{\mathrm{kHz}}
\newcommand{\GHz}{\mathrm{GHz}}
\newcommand{\msec}{\mathrm{ms}}
\newcommand{\musec}{\mathrm{\mu s}}
\newcommand{\nsec}{\mathrm{ns}}
\newcommand{\kmh}{\mathrm{km/h}}
\newcommand{\bps}{\mathrm{bit/s}}
\newcommand{\Mbps}{\mathrm{Mbit/s}}

\newcommand{\BER}{\mathrm{BER}}                % BER
\newcommand{\PER}{\mathrm{PER}}                % PER
\newcommand{\SNR}{\mathrm{SNR}}                % SNR
\newcommand{\SNRDFE}{\mathrm{\textsf{SNR}}}   % SNR f\"{u}r DFE
\newcommand{\SNRFB}{\mathrm{\textsf{SNR}}_{\mathrm{FB}}}     % SNR des FB channels
\newcommand{\SQNR}{\mathrm{\textsf{SQNR}}}              % SQNR
\newcommand{\CIR}{\mathrm{CIR}}                % CIR
\newcommand{\SER}{\mathrm{SER}}                % SER

\newcommand{\evecR}{\evec_{r}}
\newcommand{\evecT}{\evec_{t}}

\newcommand{\FBdelay}{\tau}           % FB delay

\newcommand{\rBF}{\text{rBF}}
\newcommand{\STrBF}{\text{STrBF}}
\newcommand{\heq}{h^\text{eq}}
\newcommand{\heqsupind}[2]{h^{\text{eq}, #1 }_{ #2 }}
\newcommand{\heqovl}{\ovl{h}^{^\text{eq}\ast}}

\newcommand{\BERaxis}{$\mathrm{BER} \quad \longrightarrow$}
\newcommand{\PERaxis}{$\mathrm{PER} \quad \longrightarrow$}
\newcommand{\ENaxis}{$10\log_{10}(E_b/{\cal N}_0) \quad [\dB] \quad \longrightarrow$}

%========= Abk\"{u}rzungen f\"{u}r Signalnamen (allgemein)
\newcommand{\dsig}[2]{ #1 [ #2 ] }              % zeitdiskretes Signal #1 von [#2]
\newcommand{\dsigind}[3]{ #1_{#3} [ #2 ] }      % zeitdiskretes Signal #1 von [#2] mit Index #3
\newcommand{\dsigc}[2]{ #1^{\ast} [ #2 ] }      % conj. compl. zeitdiskretes Signal #1 von [#2]
\newcommand{\dsigindc}[3]{ #1_{#3}^{\ast}[#2]}  % conj. compl. zeitdiskretes Signal #1 von [#2] mit Subindex #3

%========= Leistungsdichtespektrum
\newcommand{\clds}[2]{\Phi_{#1}(#2)}                              % LDS eines zeitkontinuierlichen Signals
\newcommand{\mclds}[2]{\overline{\Phi}_{#1}(#2)}                  % mittleres LDS eines zeitkontinuierlichen Signals
\newcommand{\dlds}[1]{\Phi_{#1}\left({\rm e}^{j 2\pi f T}\right)} % LDS eines zeitd. Signals

%========= Spektren
\newcommand{\dfreq}[1]{#1({\rm e}^{j 2\pi f T})}                  % Spektrum eines zeitd. Signals #1
\newcommand{\dfreqn}[1]{#1({\rm e}^{j 2\pi f})}                  % dfreq normiert #1
\newcommand{\dfreqind}[2]{ #1_{#2} ( {\rm e}^{j 2\pi f T} ) }     % Spektrum eines zeitd. Signals #1 mit Index #2

%========= AKF
\newcommand{\dakf}[2]{\varphi_{#1}[#2]}         % AKF eines zeitdiskreten Signals

%========= Z-Transformation
\newcommand{\zt}[1]{#1(z)}                       % z-Transf. einer Variablen #1
\newcommand{\ztind}[2]{#1_{#2}(z)}               % z-Transf. einer Variablen #1 mit Index #2
\newcommand{\ztc}[1]{#1^\ast(1/z^{\ast})}        % z-Transf. einer Variablen #1 (conjugate complex and time reversed)
\newcommand{\ztindc}[2]{#1_{#2}^\ast(1/z^{\ast})}% z-Transf. einer Variablen #1 (conjugate complex and time reversed) mit Index #2
\newcommand{\ztindsup}[3]{#1_{#2}^{#3}(z)}      % z-Transf. einer Variablen #1 mit Index #2 hoch #3
\newcommand{\ztindsupc}[3]{#1_{#2}^{\ast#3}(1/z^{\ast})}% z-Transf. einer Variablen #1 (conjugate complex and time reversed) mit Index #2 hoch #3
\newcommand{\ztm}[1]{\mathrm{\mathbf{#1}}(z)}    % z-Transf. eines Vektors/Matrix #1
\newcommand{\ztmind}[2]{\mathrm{\mathbf{#1}}_{#2}(z)}% z-Transf. eines Vektors/Matrix #1 mit Index #2
\newcommand{\ztmindsup}[3]{\mathrm{\mathbf{#1}}_{#2}^{#3}(z)}% z-Transf. eines Vektors/Matrix #1 mit Index #2 hoch #3

\newcommand{\ztcm}[1]{\mathrm{\mathbf{#1}}^{\hermitsch}(1/z^{\ast})} % z-Transf. einer Matrix #1 (conjugate complex and time reversed)
\newcommand{\ztcmind}[2]{\mathrm{\mathbf{#1}}_{#2}^{\hermitsch}(1/z^{\ast})}% z-Transf. eines Vektors/Matrix #1 mit Index #2 (conjugate complex and time reversed)
\newcommand{\ztdakf}[1]{\Phi_{#1}(z)}            % z-Transf. einer zeitdiskreten AKF

%========= Vektoren und Matrizen (allgemein)
% zeitdiskret:
\newcommand{\dma}[2]{\boldsymbol{\mathrm{#1}}[#2]}  % vector/matrix #1 of [#2]
\newcommand{\dmaind}[3]{\boldsymbol{\mathrm{#1}}_{#3}[#2]} % vector/matrix #1 of [#2] with index #3
\newcommand{\dmasup}[3]{\boldsymbol{\mathrm{#1}}^{#3} [ #2] } % vector/matrix #1 of [#2] with superscript #3
\newcommand{\dmaindsup}[4]{\boldsymbol{\mathrm{#1}}_{#3}^{#4} [ #2] } % vector/matrix #1 of [#2] with index #3 and superscript #4
\newcommand{\dmaH}[2]{\boldsymbol{\mathrm{#1}}^{\hermitsch}[#2]}  % vector/matrix #1 of [#2] hermitsch
\newcommand{\dmaindH}[3]{\boldsymbol{\mathrm{#1}}_{#3}^{\hermitsch}[#2]} % vector/matrix #1 of [#2] with index #3 hermitsch
\newcommand{\dmaT}[2]{\boldsymbol{\mathrm{#1}}^{\trsp}[#2]}  % vector/matrix #1 of [#2] transposed
\newcommand{\dmaindT}[3]{\boldsymbol{\mathrm{#1}}_{#3}^{\trsp}[#2]} % vector/matrix #1 of [#2] with index #3 transposed

\newcommand{\Km}[3]{#1_{#2#3}}  % Korrelationsmatrix

% kont.:
\newcommand{\maof}[2]{\mathrm{\mathbf{#1}}(#2)} % vector/matrix #1 of (#2)
\newcommand{\maofind}[3]{\mathrm{\mathbf{#1}}_{#3}(#2)} % vector/matrix #1 of (#2) with index #3
\newcommand{\maofsup}[3]{\mathrm{\mathbf{#1}}^{#3}(#2)} % vector/matrix #1 of (#2) with superscript #3
\newcommand{\maofindsup}[4]{\mathrm{\mathbf{#1}}_{#3}^{#4}(#2)} % vector/matrix #1 of (#2) with index #3 and superscript #4
\newcommand{\maofindH}[3]{\mathrm{\mathbf{#1}}_{#3}^{\hermitsch}(#2)} % hermitian vector/matrix #1 of #2 with index #3
%\newcommand{\ma}[1]{\boldsymbol{\mathrm{#1}}} % Matrix oder Vektor (boldmath)

%========= Vektoren % Matrizen von a - z
\newcommand{\avec}{\mathrm{\mathbf{a}}}
\newcommand{\bvec}{\mathrm{\mathbf{b}}}
\newcommand{\cvec}{\mathrm{\mathbf{c}}}
\newcommand{\dvec}{\mathrm{\mathbf{d}}}
\newcommand{\evec}{\mathrm{\mathbf{e}}}
\newcommand{\fvec}{\mathrm{\mathbf{f}}}
\newcommand{\gvec}{\mathrm{\mathbf{g}}}
\newcommand{\hvec}{\mathrm{\mathbf{h}}}
\newcommand{\ivec}{\mathrm{\mathbf{i}}}
\newcommand{\lvec}{\mathrm{\mathbf{l}}}
\newcommand{\mvec}{\mathrm{\mathbf{m}}}
\newcommand{\rvec}{\mathrm{\mathbf{r}}}
\newcommand{\svec}{\mathrm{\mathbf{s}}}
\newcommand{\tvec}{\mathrm{\mathbf{t}}}
\newcommand{\nvec}{\mathrm{\mathbf{n}}}
\newcommand{\pvec}{\mathrm{\mathbf{p}}}
\newcommand{\uvec}{\mathrm{\mathbf{u}}}
\newcommand{\vvec}{\mathrm{\mathbf{v}}}
\newcommand{\wvec}{\mathrm{\mathbf{w}}}
\newcommand{\xvec}{\mathrm{\mathbf{x}}}
\newcommand{\yvec}{\mathrm{\mathbf{y}}}
\newcommand{\zvec}{\mathrm{\mathbf{z}}}
\newcommand{\Nullvec}{\mathrm{\mathbf{0}}}
\newcommand{\Onemat}{\mathrm{\mathbf{1}}}
\newcommand{\Amat}{\mathrm{\mathbf{A}}}
\newcommand{\Bmat}{\mathrm{\mathbf{B}}}
\newcommand{\Cmat}{\mathrm{\mathbf{C}}}
\newcommand{\Dmat}{\mathrm{\mathbf{D}}}
\newcommand{\Emat}{\mathrm{\mathbf{E}}}
\newcommand{\Fmat}{\mathrm{\mathbf{F}}}
\newcommand{\Gmat}{\mathrm{\mathbf{G}}}
\newcommand{\Hmat}{\mathrm{\mathbf{H}}}
\newcommand{\Imat}{\mathrm{\mathbf{I}}}
\newcommand{\Jmat}{\mathrm{\mathbf{J}}}
\newcommand{\Kmat}{\mathrm{\mathbf{K}}}
\newcommand{\Mmat}{\mathrm{\mathbf{M}}}
\newcommand{\Nmat}{\mathrm{\mathbf{N}}}
\newcommand{\Omat}{\mathrm{\mathbf{O}}}
\newcommand{\Pmat}{\mathrm{\mathbf{P}}}
\newcommand{\Qmat}{\mathrm{\mathbf{Q}}}
\newcommand{\Rmat}{\mathrm{\mathbf{R}}}
\newcommand{\Smat}{\mathrm{\mathbf{S}}}
\newcommand{\Tmat}{\mathrm{\mathbf{T}}}
\newcommand{\Umat}{\mathrm{\mathbf{U}}}
\newcommand{\Vmat}{\mathrm{\mathbf{V}}}
\newcommand{\Wmat}{\mathrm{\mathbf{W}}}
\newcommand{\Xmat}{\mathrm{\mathbf{X}}}
\newcommand{\Ymat}{\mathrm{\mathbf{Y}}}
\newcommand{\Zmat}{\mathrm{\mathbf{Z}}}

\newcommand{\corm}{\Rmat}
\newcommand{\covm}{\Cmat}

\newcommand{\Thetavec}{\mathrm{\boldsymbol{\Theta}}}
\newcommand{\thetavec}{\mathrm{\boldsymbol{\theta}}}
\newcommand{\gammavec}{\mathrm{\boldsymbol{\gamma}}}
\newcommand{\Lambdamat}{\mathrm{\mathbf{\Lambda}}}
\newcommand{\Phimat}{\mathrm{\mathbf{\Phi}}}
\newcommand{\phivec}{\mathrm{\boldsymbol{\varphi}}}

%========= Calligraphische Buchstaben
\newcommand{\Acall}{\mathcal{A}}
\newcommand{\Ccall}{\mathcal{C}}
\newcommand{\Lcall}{\mathcal{L}}
\newcommand{\Ncall}{\mathcal{N}}
\newcommand{\Rcall}{\mathcal{R}}
\newcommand{\Scall}{\mathcal{S}}





%========= Umgebungen
% argmin: % 1. Parameter: Abstand der Variable unterhalb von 'argmax'
%           2. Parameter: Variable
\newcommand{\argmin}[2]{\! \!
    \begin{array}[t]{c}
    \displaystyle {\rm argmin} \\[#1]
    \scriptstyle #2
    \end{array} \!
    }


% argmax: % 1. Parameter: Abstand der Variable unterhalb von 'argmax'
%           2. Parameter: Variable
\newcommand{\argmax}[2]{\! \!
    \begin{array}[t]{c}
    \displaystyle {\rm argmax} \\[#1]
    \scriptstyle #2
    \end{array} \!
    }
\newcommand{\myexample}[1]{
    \begin{quote} \hspace*{-2.5em}\textbf{Example: \line(1,0){320}} \\
    #1
    \\\line(1,0){355}
    \end{quote}
    }

%% How to get an unnumbered footnote?
%% \blfootnote instead of \footnote
%\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}

% Command for rendering an unnumbered footnote
\makeatletter
\long\def\unmarkedfootnote#1{{\long\def\@makefntext##1{##1}\footnotetext{#1}}}
\makeatother


%========= a "watermark"/EPS graphics behind text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro         :   \BackgroundEPS{filename}{tx}{ty}{s}
%-----------------------------------------------------------------------
% Description   :   Display an EPS file in the background of the
%                   current page.
%-----------------------------------------------------------------------
% Author        :   Bernard Desruisseaux (bernard@XYZZYcs.mcgill.ca)
%-----------------------------------------------------------------------
% Usage         :   \BackgroundEPS{pic.eps}{80}{100}{2}
%                   \BackgroundEPS{"`gunzip -c pic.eps.gz"}{80}{100}{2}
%                   \BackgroundEPS{"`zcat pic.eps.Z"}{80}{100}{2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\BackgroundEPS#1#2#3#4{%
    \special{ps: @beginspecial @setspecial initmatrix
                0.9 setgray #2 #3 translate #4 dup scale}
    \special{ps: plotfile #1}
    \special{ps: @endspecial}
}

